gazel: Supporting Source Code Edits in Eye-Tracking Studies

Eye tracking tools are used in software engineering research to study various software development activities. However, a major limitation of these tools is their inability to track gaze data for activities that involve source code editing. We present a novel solution to support eye tracking experiments for tasks involving source code edits as an extension of the iTrace community infrastructure. We introduce the iTrace-Atom plugin and gazel -- a Python data processing pipeline that maps gaze information to changing source code elements and provides researchers with a way to query this dynamic data. iTrace-Atom is evaluated via a series of simulations and is over 99% accurate at high eye-tracking speeds of over 1,000Hz. iTrace and gazel completely revolutionize the way eye tracking studies are conducted in realistic settings with the presence of scrolling, context switching, and now editing. This opens the doors to support many day-to-day software engineering tasks such as bug fixing, adding new features, and refactoring.

==> Problem.tex <==
\label{sec:problem}

% \begin{figure*}[h]
% \centering
%     \includegraphics[width=.9\linewidth]{challenges.png}
%   \caption{Challenges of tracking gazes on edited source code}
%   \label{fig:edit-challenge}
% \end{figure*}

\subsection{Supporting Source Code Edits}
\subsubsection{Capturing Edit Information}
Supporting source code editing is a non-trivial challenge. In order to generate correct gaze information, eye tracking data provided from the eyetracker at time $t_n$ needs to be mapped to the appropriate source code elements for the snapshot of the code that was being viewed at the same time $t_n$. All versions of the source code need to be captured and parsed in order to generate correct gaze information. 
%One option is to save a snapshot of the code periodically (e.g. every second, or triggered by an edit), and use timestamps of gaze data to map to the corresponding source code version.  This solution is time and memory inefficient: the number of files would grow with the time of length of the experiment, number of edits made, and number of files in the project. Furthermore, every snapshot file needs to be parsed with a language parser in order to map gaze data, adding on unnecessary computation time.

\subsubsection{Tracking Tokens and Gazes}
Another challenge is tracking how gazes change as syntactic elements are edited, inserted, or deleted from a file.  Figure~\ref{fig:edit-challenge} contains two snapshots of the a source code file, snapshot 1 is the original file and snapshot 2 has an new line inserted on line 66. Three gaze fixations recorded on Snapshot 1 are displayed as yellow circles on the figure. Fixation 1 is recorded on line 64, fixation 2 on line 68, and fixation 3 on line 71. 

Current solutions assume the text at a specific line and column is static, and resolve syntactic tokens by parsing the source file. However, when a new line is inserted on line 66, fixation 2 and 3 are still mapped to lines 68 and 71. However, the syntactic token under the fixation has changed. Fixation 3 was correctly mapped on to  the identifier 'frequency', but with the edit, is now mapped to white space. A viable solution needs to keep track of all edits, and resolve gazes the correct syntactic tokens.

\subsection{Supporting High Speed Eyetrackers}
A current challenge for existing eye tracking plugins is the high latency of API calls within the IDE prevents real time gaze and textual analysis at the data sampling rate of high-speed eye trackers. This is because IDEs like Visual Studio, do not expose direct APIs for solving line and column indices and when data sampling rates exceed the API call time, gazes from the eyetracker are not captured by the plugin. Support for high speed eye trackers is crucial for software engineering researchers to use different metrics of gaze information, such as saccades, and improved precision and accuracy for metrics already in use, like fixations and dwell time.

One way that researchers have addressed this problem is through \dejavu \cite{dejavu}, which moves any real-time analysis being done by the plugin into an offline tool which which allows ample time for the IDE to map gaze point positions to the appropriate file, line and columns. 
However, software engineering researchers often require quick analysis of eye tracking data for use in post-experiment surveys to gain more insight into comprehension processes or unexpected behavioral patterns. Quick real-time resolution of x,y coordinates is needed for this scenario.







